An Empirical Analysis of Community and Coding Patterns in OSS4SG vs. Conventional OSS

Open Source Software for Social Good (OSS4SG) projects aim to address critical societal challenges, such as healthcare access and community safety. Understanding the community dynamics and contributor patterns in these projects is essential for ensuring their sustainability and long-term impact. However, while extensive research has focused on conventional Open Source Software (OSS), little is known about how the mission-driven nature of OSS4SG influences its development practices. To address this gap, we conduct a large-scale empirical study of 1,039 GitHub repositories, comprising 422 OSS4SG and 617 conventional OSS projects, to compare community structure, contributor engagement, and coding practices. Our findings reveal that OSS4SG projects foster significantly more stable and "sticky" (63.4%) communities, whereas conventional OSS projects are more "magnetic" (75.4%), attracting a high turnover of contributors. OSS4SG projects also demonstrate consistent engagement throughout the year, while conventional OSS communities exhibit seasonal fluctuations. Additionally, OSS4SG projects rely heavily on core contributors for both code quality and issue resolution, while conventional OSS projects leverage casual contributors for issue resolution, with core contributors focusing primarily on code quality.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> acknowledgment.tex <==
% Acknowledgment section
% This file is not currently used in the main document
% The acknowledgment is included directly in conclusion.tex



==> old_results.tex <==
\begin{table}[htbp]
\centering
\caption{Overview of Collected Raw Metrics for Each Project and Their Use in Research Questions.}
\label{tab:collected-data}
\small
\begin{tabular}{p{1.5cm}|p{5cm}|p{1cm}}
\hline
\textbf{Category} & \textbf{Collected Metrics} & \textbf{Research Question} \\ \hline
\textbf{Project Metrics}  
& Programming Languages, Project Start Date, Date of Last Contribution, Project Lifespan, Star Count, Subscriber Count, Fork Count, Open Issue Count, Closed Issue Count, Open Pull Request Count, Closed Pull Request Count, Merged Pull Request Count 
& RQ1 \\ \hline
\textbf{Developer Metrics}  
& Total Contributor Count, Core Contributor Count, Commit Count, Commit Additions, Commit Deletions, Average Commit Message Length 
& RQ1, RQ2 \\ \hline
\textbf{Code Metrics}  
& Total Lines of Code, Total Character Count, Comment Line Count, Non-Comment Line Count, Code-to-Comment Ratio, Code Character Count, Comment Character Count, Code-to-Comment Character Ratio, Repository Size (Megabytes), README Character Count, Qodana Scan Results (Issue Severity Levels: Critical, High, Moderate, Low), Total Issue Count, Understand SciTools Code Metrics 
& RQ1, RQ3 \\ \hline
\end{tabular}
\end{table}
% Add this package to your document preamble if not already present:
% \usepackage{xcolor}








\begin{table}[htbp]
\centering
\caption{Mann--Whitney U Test Results for Project and Community Metrics. We show statistically significant differences (green cells), effect size (L/M/S), and (OSS4SG/OSS -1).}
\label{tab:project_metrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c}
\hline
\textbf{Metric} & \textbf{p-value} & \textbf{Effect Size} & \textbf{OSS4SG/OSS Ratio} \\
\hline

\rowcolor{gray!20}\multicolumn{4}{l}{\textbf{Popularity}} \\ \hline
Star Count              & \cellcolor{green!20}0.00  & L & -0.80 \\ \hline
Subscriber Count        & \cellcolor{green!20}0.00  & L & -0.70 \\ \hline
Fork Count              & \cellcolor{green!20}0.00  & L & -0.76 \\ \hline

\rowcolor{gray!20}\multicolumn{4}{l}{\textbf{Community Composition}} \\ \hline
Contributor Count       & 0.58                        & S & -0.45 \\ \hline
Core Contributor Count  & \cellcolor{green!20}0.00  & M & 1.80 \\ \hline

\rowcolor{gray!20}\multicolumn{4}{l}{\textbf{Contributions}} \\ \hline
Commit Count            & \cellcolor{green!20}0.00  & M & 0.90 \\ \hline
Open PR Count           & 0.15                        & S & -0.20 \\ \hline
Closed PR Count         & \cellcolor{green!20}0.00  & M & 2.80 \\ \hline
Merged PR Count         & 0.15                        & S & 0.15 \\ \hline
Open Issue Count        & 0.11                        & S & 0.10 \\ \hline
Closed Issue Count      & \cellcolor{green!20}0.00  & S & 2.00 \\ \hline
Average PR Resolution Time & \cellcolor{green!20}0.00  & S & -0.31 \\ \hline

\rowcolor{gray!20}\multicolumn{4}{l}{\textbf{Readability}} \\ \hline
Average Commit Message Length & \cellcolor{green!20}0.00 & S & 0.50 \\ \hline
Comment Line Count       & 0.98                        & S & -0.42 \\ \hline
Comment Character Count  & 0.57                        & S & 0.92 \\ \hline
Code-to-Comment Ratio    & 0.07                        & S & 0.78 \\ \hline
Code-to-Comment Character Ratio & 0.60               & S & -0.30 \\ \hline

\rowcolor{gray!20}\multicolumn{4}{l}{\textbf{Project Size}} \\ \hline
Total Lines of Code      & 0.34                        & S & -0.01 \\ \hline
Non-Comment Line Count   & 0.31                        & S & 0.16 \\ \hline
Total Character Count    & 0.19                        & S & 0.18 \\ \hline
Code Character Count     & 0.17                        & S & 0.31 \\ \hline
\textsc{Readme} Character Count & 0.29                & S & -0.35 \\ \hline
Repository Size (MB)     & \cellcolor{green!20}0.00   & S & -0.08 \\ \hline

\end{tabular}%
}
\end{table}





%In this section, we present the empirical findings for each research question, organized in the same order as described in our methodology. Figures~\ref{fig:rq1_barplot}, \ref{fig:rq2_scatter}, \ref{fig:rq2mid}, \ref{fig:rq3_timeseries}, and \ref{fig:rq4_commitpattern} illustrate the key comparisons. All statistical results are referenced in the text.

\subsection{RQ1: \mohamed{To what extent do  project attributes differ between standard Open Source Software (OSS) projects and OSS for Social Good (OSS4SG) projects?}}

Figure~\ref{fig:rq1_barplot} reveals that OSS4SG projects have a substantially higher proportion of core contributors, commits, and merged pull requests. In contrast, OSS projects exhibits higher values for stars, forks, and subscribers. \mohamed{One notable observations regarding the project size metrics is that OSS4SG projects have lengthier comments compared to OSS projects (1.8 times longer). This difference may reflect stronger dynamics within the OSS4SG, as contributors might prioritize clear communication and documentation. } 
%_________________
% topic sentence (What is the main take away?)


%OSS4SG leads in core contributor engagement while OSS projects are more popular.
A descriptive comparaison of OSS4SG and OSS projects shows that OSS4SG projects have higher core contributor engagement, while OSS projects are more popularity. 

%eventhough OSS projects have more contributors, OSS4SG projects have more core contributors and show more contribution activity.. 
Despite OSS projects having on average a larger contributor base than OSS4SG projects, OSS4SG have XX more core contributors. In addition, OSS4SG projects display higher proportion of contributions including commits (XX more than OSS projects) and closed PRs (XX more). This may be attributed to the social mission of OSS4SG, which might attracts contributors who are deeply committed to the project and strongly aligned with its goals. In addition... 

% different than that, OSS project are more popular with Stars (), forks ()
% Write about popularity metrics similar to what I have written above
In contrast, OSS projects are on average XX.....

%
%____________
%Notably, 6.96\% of contributors in OSS4SG are active in multiple projects within OSS4SG, compared to only 2.41\% in OSS, while cross-category participation remains minimal at approximately 1\%.

\mohamed{I’ve added additional columns that are related to the project size, such as the number of characters and lines of code, and made the figure more readable.}





\mohamed{I have add the following plot that represent the distributions of the contributors}


\mohamed{Figure \ref{fig:rq1_ContDist} illustrates the differences in contributors’ dynamics between OSS and OSS4SG projects. While OSS has a larger overall number of contributors, approximately 1.2 times the number of contributors to OSS4SG, OSS4SG contributors are three times more active in other projects compared to OSS contributors within the same category. For the distribution of contributors across 2, 3, and 4+ projects, the percentages are nearly identical between OSS and OSS4SG, showing no significant difference. However, the higher likelihood of OSS4SG contributors participating in multiple projects overall might be explained by the mission-driven nature of these projects, which could inspire contributors to extend their efforts across other projects that might have the same mission.}



\begin{tcolorbox}[colback=gray!10, colframe=black]
\textbf{RQ1 Answer:} \\
OSS4SG projects exhibit over 1.5 times higher counts of core contributors, commits, closed issues, and merged pull requests compared to OSS. 
OSS projects, however, display higher overall popularity metrics (stars and forks) but less concentrated core engagement. Additionally, 6.96\% of OSS4SG contributors participate in multiple projects (versus 2.41\% in OSS), while only about 1\% overlap between the two categories.
\end{tcolorbox}







\subsection{RQ2: Stability of OSS4SG vs.\ OSS (Newcomers and Leavers)}
We assessed project stability by segmenting each repository’s lifespan into quartile-based stages \cite{wang2012survival}. Figure~\ref{fig:rq2_scatter} presents a KDE plot of join versus leave rates across all stages, using a four-quadrant model (Attractive, Unstable, Stable, Unattractive).

\shayan{How do we measure join/leave? we should clearly define this as I think: join/leave only has meaning on core contributors because occasional contributors can be one committer for example.}
\mohamed{Here we calculated the join/leave rate for each project that includes the non-core contributors. But I think you are correct. I will re do them but having only the core contributors in mind. }

\noindent
\textbf{Key Observations (All Stages):}
\begin{itemize}
    \item Approximately 63.3\% of OSS4SG projects are classified as stable, whereas 75\% of OSS projects fall into the unstable quadrant.
\end{itemize}


\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{figures/RQ2_early_and_mid-late.png}
\caption{KDE plot of join vs.\ leave rates. for early and mid-late stages (merged duo to being very similar).}
\label{fig:rq2mid}
\end{figure}



Figure~\ref{fig:rq2mid} further dissects these patterns into early, mid, and late stages:
\begin{itemize}
    \item \textbf{Early Stage (0--7.421~years):} 59.3\% of OSS4SG projects are stable, compared to 74\% of OSS projects being unstable.
    \item \textbf{Mid Stage (7.421--9.115~years):} OSS4SG projects maintain higher stability (44\%) versus 30.9\% in OSS.
    \item \textbf{Late Stage (9.115--10.923~years):} 48.7\% of OSS4SG projects remain stable, in contrast to 34.3\% for OSS, with differences diminishing relative to earlier stages.
\end{itemize}

Statistical tests (Mann–Whitney U, <0.01$ with medium effect size) confirm significantly lower leave rates and higher stability in OSS4SG during the early and mid stages. Late-stage differences, however, were not statistically significant at $p<0.05$ following Bonferroni corrections.

~\shayan{I think a scott-knott test could be more useful here as it can rank and cluster all data together. instead of having multiple pairwise U tests.}
\mohamed{I just looked into the Scott-Knott test and it seems good for our project. I will apply it to our data and add its results.}
~\shayan{I think it is important here to differentiate the types of developers in the leave/join analysis. We can't put them all in the same bucket.}
\mohamed{so we split our finding into two categories one for the core and the other for non-core?}\shayan{I believe so}

\begin{tcolorbox}[colback=gray!10, colframe=black]
\textbf{RQ2 Answer:} \\
Overall, OSS4SG projects demonstrate greater stability. In the early stage, 59.3\% are stable compared to only 26\% of OSS projects. For mid to late stages, stability in OSS4SG ranges from 44\% to 48.7\%, while OSS projects consistently exhibit lower stability (30.9\%--34.3\%).
\end{tcolorbox}



\subsection{RQ3: Turnover and Retention over Time}
Figure~\ref{fig:rq3_timeseries} plots the average monthly join and leave rates over a project’s lifecycle. OSS4SG projects maintain a relatively constant join rate of around 20\%, while OSS projects start with high join rates that decline over time. Similarly, OSS4SG leave rates remain stable at approximately 15\%, whereas OSS projects initially exhibit nearly double the leave rate, which decreases as projects mature.~\shayan{I think rather than using two separate time series plots (leave plot and join plot), we can combine them into a single plot by normalizing the number of joins by the number of leaves (i.e., joins/leaves). It is important to compare the two time series—one for OSS and another for OSS4SG—across different phases to assess whether there is a significant difference in the joining ratio.}~\shayan{If this analysis is for core contributors, we can repeat and report results bu condidering different types of contributors.}
 







\noindent
\textbf{Key Observations:}
\begin{itemize}
    \item \emph{Join Rates:} OSS4SG projects maintain a steady join rate (~20\%) across all stages, whereas OSS projects exhibit a significant drop over time (statistically significant differences in the early stage, Mann–Whitney, $p<0.01$).
    \item \emph{Leave Rates:} OSS4SG projects have a consistent leave rate (~15\%), while OSS projects start with nearly twice the leave rate and gradually decrease (Wilcoxon, $p<0.01$, medium effect size).
\end{itemize}
~\shayan{It is important to discuss our findings at the end of each RQ and justify the implications of our findings.}

\begin{tcolorbox}[colback=gray!10, colframe=black]
\textbf{RQ3 Answer:} \\
OSS4SG projects exhibit more consistent contributor retention across all life stages, while OSS projects experience high turnover in early stages that stabilizes later.
\end{tcolorbox}

\subsection{RQ4: Commit Frequency Among Core vs.\ Non-Core Contributors}
We aggregated a total of \textbf{2,219,796} commits, with \textbf{580,144} from OSS and \textbf{1,639,652} from OSS4SG. Core contributors (those producing the top 80\% of commits~\cite{Ferreira2020}) in OSS4SG display consistent, high-level activity throughout the year. In contrast, OSS core contributors show pronounced seasonal fluctuations. The gap between core and non-core contributor activity is also much more pronounced in OSS4SG projects, indicating that core contributors play a critical role in maintaining stability.

\noindent

\textbf{Key Observations.}
\begin{itemize}
    \item \emph{Core Contributors:} OSS4SG core contributors exhibit consistently high working capacity throughout the year, maintaining stable activity levels. By contrast, OSS core contributors demonstrate seasonal patterns, with activity fluctuating significantly.
    \item \emph{Core vs.\ Non-Core Disparity:} OSS4SG projects show a notable disparity~\shayan{Claims should be supported by numerical evidence; words like "notable" without proper statistical support can be misleading. It is important to provide concrete metrics or statistical analysis to substantiate such statements} between core and non-core contributor patterns, with core contributors driving project stability. In OSS, this gap is much smaller, indicating less differentiation in roles.
    \item \emph{Non-Core Contributors:} Non-core contributors in both OSS4SG and OSS display fluctuating activity levels, with clear instability. A prominent spike in October, corresponding to Hacktoberfest, highlights their seasonal influence on project activity.
    \item \emph{Impact on Stability:} OSS4SG core contributors significantly contribute to overall project stability, underscoring their critical role. OSS core contributors, however, do not exhibit the same level of consistency or influence on project stability.
\end{itemize}

\noindent
\textbf{Clustering Insights.}
We clustered weekly commit series using Dynamic Time Warping (DTW) and identified two main clusters. One cluster predominantly consisted of OSS4SG core contributors, characterized by sustained and consistent weekly commits, highlighting their pivotal role in project stability. The second cluster included the remaining contributors, encompassing sporadic and less stable activity patterns. Due to the high density of data points, the resulting heatmap was difficult to interpret and thus is not included in this document.
~\shayan{We need to define why two clusters are optimal. you can use the elbow method/silhouette score}





\begin{tcolorbox}[colback=gray!10, colframe=black]
\textbf{RQ4 Answer:} \\
Among 2.22M commits, OSS4SG projects (1.64M commits) exhibit higher sustained commit activity than OSS projects (0.58M commits). OSS4SG core contributors form stable activity clusters, whereas OSS contributors show more sporadic, bursty patterns.
\end{tcolorbox}





\subsection{RQ5: Code Issues and Anti-Patterns}
Finally, we explored whether OSS4SG differs in code quality~\shayan{If we want to study the code quality, which I think is very important, we may want to adjust this RQ and use a wider range of metrics to explain code quality. There are tools to measure code quality (e.g., understand).} or recurring issues, using Qodana scans.



\noindent
\textbf{Key Observations.}
\begin{itemize}
    \item \emph{Average Problem Counts:} OSS projects show about 1,663 total problems on average, whereas OSS4SG reports around 2,407 total problems. OSS4SG also has more high-severity issues, possibly due to having less contributors.
    \item \emph{Leading Issue Types:} 
    \begin{itemize}
        \item \textbf{OSS} top issues: XAML errors, Javadoc problems, operator coercion, PEP~8 naming, ESLint warnings.
        \item \textbf{OSS4SG} top issues: comma expressions, ESLint, operator coercion, PEP~8 naming, unused symbols.
    \end{itemize}
    \item Some items (e.g., ESLint, PEP~8) overlap, suggesting common Python and JavaScript usage in both. Others (e.g., XAML errors in OSS vs.\ comma expressions in OSS4SG) imply domain or language differences.
\end{itemize}

\noindent



\begin{tcolorbox}[colback=gray!10,colframe=black]
\textbf{RQ5 Answer:} 
OSS4SG averages \emph{2{,}407} Qodana-flagged issues vs.\ \emph{1{,}663} in OSS, commonly including ESLint, PEP\,8, and operator coercion. OSS-specific problems (e.g., XAML errors) and OSS4SG’s comma expressions suggest language/domain differences rather than uniform quality gaps.
\end{tcolorbox}


==> tables/Qodana_metrics_def_table_.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\caption{Qodana severity classes.}
\begin{tabularx}{\columnwidth}{X}
\toprule

\textbf{Critical}: Must-fix defects. \\
\textit{Example:} In C++, dereferencing a pointer that was never initialised can crash the program (null-pointer dereference). \\ \midrule
\textbf{High}: Likely bugs or major smells. \\
\textit{Example:} A Java method annotated \emph{@NonNull} nevertheless returns \emph{null}, risking a run-time null-pointer exception. \\ \midrule
\textbf{Moderate}: Maintainability or style issues. \\
\textit{Example:} Two identical 12-line blocks appear in different functions, increasing future maintenance effort. \\ \bottomrule
\end{tabularx}

\label{tab:qodana_severities}
\end{table}

==> tables/Qualty_metrics_clusters.tex <==
\begin{table}[h]
\centering
\caption{Median quality Metrics by Cluster for OSS and OSS4SG~\shayan{can we have cohesion and coupling metrics too?}}
\label{tab:median_complexity}
\scriptsize
\begin{tabular}{@{}l@{}}
\toprule
\multicolumn{1}{c}{\textbf{Cyclomatic Complexity:}} \\
\midrule
\textbf{Cluster 1:} OSS: \textbf{P1} (0.17), \textbf{P0} (0.24); OSS4SG: \textbf{P0} (0.15), \textbf{P2} (0.18), \textbf{P3} (0.18) \\
\midrule
\textbf{Cluster 2:} OSS: \textbf{P2} (0.38); OSS4SG: \textbf{P1} (0.29) \\
\midrule
\textbf{Cluster 3:} OSS: \textbf{P3} (0.56); OSS4SG: -- \\
\midrule
\multicolumn{1}{c}{\textbf{Nesting Complexity:}} \\
\midrule
\textbf{Cluster 1:} OSS: \textbf{P0} (0.23), \textbf{P2} (0.24), \textbf{P1} (0.31); OSS4SG: \textbf{P0} (0.13), \textbf{P2} (0.28), \textbf{P1} (0.31) \\
\midrule
\textbf{Cluster 2:} OSS: \textbf{P3} (0.51); OSS4SG: \textbf{P3} (0.37) \\
\bottomrule
\end{tabular}
\end{table}

==> tables/quality_metric_Q.tex <==
\begin{table}[ht]
\small
\centering
\begin{tabular}{lccccc}
\toprule
 & Critical & High & Moderate & Low & Total \\
\midrule
OSS    & 65.40   & 166.49   & 130.89   & 0.00   & 362.78  \\
OSS4SG & 73.91   & 123.68   & 104.08   & 0.00   & 301.67  \\
\bottomrule
\end{tabular}
\caption{Issues per 10M Code Characters for OSS and OSS4SG}
\label{tab:issues}
\end{table}

==> tables/quality_understand_metrics_table_withotuh_qodana.tex <==
\begin{table*}[htbp]
\centering
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{ll *{6}{r} *{2}{r} *{6}{r}}
\toprule
\multirow{2}{*}{\textbf{Project}} &
\multirow{2}{*}{\textbf{Pattern}} &
\multicolumn{6}{c}{\textbf{Lack of Complexity} (higher $\uparrow$)} &
\multicolumn{2}{c}{\textbf{Documentation} (higher $\uparrow$)} &
\multicolumn{6}{c}{\textbf{Organization} (higher $\uparrow$)}\\
\cmidrule(lr){3-8}\cmidrule(lr){9-10}\cmidrule(lr){11-16}
 & & \multicolumn{2}{c}{Cyclomatic} &
     \multicolumn{2}{c}{Max Nesting} &
     \multicolumn{2}{c}{Max Inheritance Tree} &
     \multicolumn{2}{c}{Ratio Comment / Code} &
     \multicolumn{2}{c}{Count Decl Method All} &
     \multicolumn{2}{c}{Count Decl Function} &
     \multicolumn{2}{c}{Count Decl Method} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}%
\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}
 &  & Rank & Median & Rank & Median & Rank & Median &
    Rank & Median & Rank & Median & Rank & Median & Rank & Median \\
\midrule
\textbf{OSS} & Declining core activity
  & \cellcolor{orange!20}3 & 0.33
  & \cellcolor{yellow!20}4 & 0.47
  & \cellcolor{yellow!20}4 & 0.78
  & \cellcolor{green!20}2 & 0.10
  & \cellcolor{yellow!20}4 & 0.16
  & \cellcolor{orange!20}3 & 0.23
  & \cellcolor{green!20}2 & 0.34 \\
 & High core activity
  & \cellcolor{blue!20}1 & 0.91
  & \cellcolor{blue!20}1 & 0.84
  & \cellcolor{blue!20}1 & 0.89
  & \cellcolor{blue!20}1 & 0.11
  & \cellcolor{blue!20}1 & 0.05
  & \cellcolor{blue!20}1 & 0.06
  & \cellcolor{blue!20}1 & 0.12 \\
 & Increasing core activity
  & \cellcolor{orange!20}3 & 0.85
  & \cellcolor{cyan!20}5 & 0.81
  & \cellcolor{cyan!20}5 & 0.87
  & \cellcolor{orange!20}3 & 0.12
  & \cellcolor{cyan!20}5 & 0.08
  & \cellcolor{orange!20}3 & 0.08
  & \cellcolor{green!20}2 & 0.14 \\
 & Low core activity
  & \cellcolor{blue!20}1 & 0.75
  & \cellcolor{blue!20}1 & 0.81
  & \cellcolor{blue!20}1 & 0.86
  & \cellcolor{blue!20}1 & 0.34
  & \cellcolor{blue!20}1 & 0.09
  & \cellcolor{blue!20}1 & 0.18
  & \cellcolor{blue!20}1 & 0.24 \\[2pt]

\textbf{OSS4SG} & Declining core activity
  & \cellcolor{green!20}2 & 0.79
  & \cellcolor{orange!20}3 & 0.65
  & \cellcolor{orange!20}3 & 0.58
  & \cellcolor{green!20}2 & 0.18
  & \cellcolor{orange!20}3 & 0.30
  & \cellcolor{green!20}2 & 0.22
  & \cellcolor{blue!20}1 & 0.37 \\
 & High core activity
  & \cellcolor{green!20}2 & 0.78
  & \cellcolor{green!20}2 & 0.71
  & \cellcolor{green!20}2 & 0.72
  & \cellcolor{blue!20}1 & 0.14
  & \cellcolor{green!20}2 & 0.25
  & \cellcolor{green!20}2 & 0.20
  & \cellcolor{blue!20}1 & 0.22 \\
 & Increasing core activity
  & \cellcolor{yellow!20}4 & 0.78
  & \cellcolor{red!20}6 & 0.75
  & \cellcolor{red!20}6 & 0.75
  & \cellcolor{cyan!20}5 & 0.35
  & \cellcolor{brown!20}7 & 0.13
  & \cellcolor{cyan!20}5 & 0.30
  & \cellcolor{orange!20}3 & 0.15 \\
 & Low core activity
  & \cellcolor{orange!20}3 & 0.73
  & \cellcolor{cyan!20}5 & 0.83
  & \cellcolor{red!20}6 & 0.82
  & \cellcolor{yellow!20}4 & 0.16
  & \cellcolor{red!20}6 & 0.11
  & \cellcolor{yellow!20}4 & 0.09
  & \cellcolor{orange!20}3 & 0.35 \\
\bottomrule
\end{tabular}}
\caption{Scott–Knott clusters and medians for selected \textit{Understand} metrics (values truncated to 2 decimal places)}
\label{tab:clustring-understand-metrics}
\end{table*}

==> tables/understand_explaining_.tex <==




\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\columnwidth}{X}
\toprule

\textbf{Cyclomatic complexity}: Counts independent execution paths. \\
\textit{Example:} A simple \emph{if/else} branch introduces two distinct paths and therefore a complexity of 2. \\ \midrule
\textbf{Max nesting level}: Deepest stack of control statements. \\
\textit{Example:} A loop that contains an \emph{if}, which in turn contains another loop, has a nesting level of 3. \\ \midrule
\textbf{Depth of inheritance tree (DIT)}: Longest inheritance chain. \\
\textit{Example:} \emph{Animal → Mammal → Dog} results in a DIT of 3, making behaviour harder to trace. \\ \midrule
\textbf{Ratio comment / code}: Comment lines divided by code lines. \\
\textit{Example:} One comment line and two code lines yield a ratio of 0.50. \\ \midrule
\textbf{Declared methods (all)}: Methods available on a class, including those it inherits. \\ \midrule
\textbf{Declared functions}: Stand-alone or free functions in a file or module, indicating functional fan-out. \\ \midrule
\textbf{Declared methods (local)}: Methods declared directly in the class (excluding inherited ones), reflecting the class’s own size. \\ \bottomrule
\end{tabularx}
\caption{Understand metrics.}
\label{tab:understand_metrics}
\end{table}
